Single Image Defocus Deblurring Using Kernel-Sharing Parallel Atrous Convolutions

This paper proposes a novel deep learning approach for single image defocus deblurring based on inverse kernels. In a defocused image, the blur shapes are similar among pixels although the blur sizes can spatially vary. To utilize the property with inverse kernels, we exploit the observation that when only the size of a defocus blur changes while keeping the shape, the shape of the corresponding inverse kernel remains the same and only the scale changes. Based on the observation, we propose a kernel-sharing parallel atrous convolutional (KPAC) block specifically designed by incorporating the property of inverse kernels for single image defocus deblurring. To effectively simulate the invariant shapes of inverse kernels with different scales, KPAC shares the same convolutional weights among multiple atrous convolution layers. To efficiently simulate the varying scales of inverse kernels, KPAC consists of only a few atrous convolution layers with different dilations and learns per-pixel scale attentions to aggregate the outputs of the layers. KPAC also utilizes the shape attention to combine the outputs of multiple convolution filters in each atrous convolution layer, to deal with defocus blur with a slightly varying shape. We demonstrate that our approach achieves state-of-the-art performance with a much smaller number of parameters than previous methods.

==> figures/experiments/fig_template.tex <==
\begin{figure*}[t]
\centering
    \def \ext {.jpg} % .jpg / .png

    %% ROW1
    \def \corl {0.42} %left
    \def \corb {0.33} %bottom
    \def \corrt {0.15} % right = left + corrt / top = bottom + corrt
    
    % \def \corls {0.8} %left
    % \def \corbs {0.72} %bottom
    % \def \corrts {0.2} % right = left + corrt / top = bottom + corrt
    \def \corls {0.85} %left
    \def \corbs {0.49} %bottom
    \def \corrts {0.15} % right = left + corrt / top = bottom + corrt
    \def \img {62\ext} % right = left + corrt / top = bottom + corrt

    \setlength\tabcolsep{0.2 pt}
    % % \def \wb {0.14}
    % % \def \ws {0.069}
    \def \wb {0.195}
    \def \ws {0.097}
    
    \begin{tabular}{lrlrlrlrlrlrlrlr}
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/Input/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/JNB/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/EBDB/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DMENet/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DPDNet/single/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DPDNet/dual/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/Ours/single/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/GT/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} \\[-0.04in]
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)},clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Input/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Input/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/JNB/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/JNB/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/EBDB/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/EBDB/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DMENet/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DMENet/\img}} &

    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/single/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/single/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/dual/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/dual/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Ours/single/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Ours/single/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/GT/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/GT/\img}}
    
    \\[-0.04in]
    \end{tabular}
  
    %% ROW2
    % \def \corl {0.043} %left
    % \def \corb {0.49} %bottom
    % \def \corrt {0.13} % right = left + corrt / top = bottom + corrt
    \def \corl {0.024} %left
    \def \corb {0.72} %bottom
    \def \corrt {0.1} % right = left + corrt / top = bottom + corrt
    
    \def \corls {0.76} %left
    \def \corbs {0.595} %bottom
    \def \corrts {0.13} % right = left + corrt / top = bottom + corrt
    \def \img {59\ext} % right = left + corrt / top = bottom + corrt
    
    \begin{tabular}{lrlrlrlrlrlrlrlr}
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/Input/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/JNB/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/EBDB/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DMENet/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DPDNet/single/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DPDNet/dual/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &    
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/Ours/single/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/GT/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} \\[-0.04in]
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Input/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Input/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/JNB/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/JNB/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/EBDB/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/EBDB/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DMENet/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DMENet/\img}} &

    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/single/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/single/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/dual/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/dual/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Ours/single/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Ours/single/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/GT/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/GT/\img}}
    
    \\[-0.04in]
    \end{tabular}
    
    %% ROW3
    \def \corl {0.00} %left
    \def \corb {0.44} %bottom
    \def \corrt {0.1} % right = left + corrt / top = bottom + corrt
    
    \def \corls {0.93} %left
    \def \corbs {0.48} %bottom
    \def \corrts {0.07} % right = left + corrt / top = bottom + corrt
    \def \img {36\ext} % right = left + corrt / top = bottom + corrt
    
    \begin{tabular}{lrlrlrlrlrlrlrlr}
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/Input/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/JNB/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/EBDB/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DMENet/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &

    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DPDNet/single/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/DPDNet/dual/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/Ours/single/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} &
    
    \multicolumn{2}{c}{
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\wb\textwidth]{data/DPDD/figures/GT/\img}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
        \draw[red,thick] ([shift={(0.01, 0.01)}]\corl, \corb) rectangle ([shift={(-0.01, -0.01)}]{\corl+\corrt}, {\corb+\corrt});
        \draw[green,thick] ([shift={(0.01, 0.01)}]\corls, \corbs) rectangle ([shift={(-0.01, -0.01)}]{\corls+\corrts}, {\corbs+\corrts});
    \end{scope}
    \end{tikzpicture}} \\[-0.04in]
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Input/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Input/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/JNB/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/JNB/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/EBDB/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/EBDB/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DMENet/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DMENet/\img}} &

    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/single/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/single/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/dual/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/DPDNet/dual/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Ours/single/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/Ours/single/\img}} &
    
    \adjustbox{width=\ws\textwidth, trim={\corl\width} {\corb\height} {\width-(\corl\width+\corrt\width)} {\height-(\corb\height+\corrt\height)}, clip,cfbox=red 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/GT/\img}} &
    \adjustbox{width=\ws\textwidth, trim={\corls\width} {\corbs\height} {\width-(\corls\width+\corrts\width)} {\height-(\corbs\height+\corrts\height)}, clip,cfbox=green 0.7pt -0.7pt}
    {\includegraphics[width=\ws\textwidth]{data/DPDD/figures/GT/\img}}
    
    \\[-0.04in]
    
    \multicolumn{2}{c}{\small{(a) Input}} &
    \multicolumn{2}{c}{\small{(b) JNB}} &
    \multicolumn{2}{c}{\small{(c) EBDB}} &
    \multicolumn{2}{c}{\small{(d) DMENet}} &
    \multicolumn{2}{c}{\small{(e) DPDNet$_{\scaleto{single}{4pt}}$}} &
    \multicolumn{2}{c}{\small{(f) DPDNet$_{\scaleto{dual}{4pt}}$}} &
    % \multicolumn{2}{c}{\small{(g) Ours$_{\scaleto{single}{4pt}}$}} &
    \multicolumn{2}{c}{\small{(g) Ours}} &
    \multicolumn{2}{c}{\small{(h) GT}}
    \\
  \end{tabular}
 \caption{Qualitative comparison on DPDD dataset \cite{Abuolaim:2020:DPDNet}.
% For each row, we show different samples in DPDD-dataset. 
Images in the first and last columns are defocused input image and ground-truth all-in-focus image, respectively. The images in between the columns are deblurring results for each method.
Images in the red and green boxes are zoomed-in cropped patches for better comparison.
Note that images in (f) are results of dual-pixel based DPDNet, where other methods including ours take only a single input at inference time. 
We refer readers to the supplementary material for more results.
  }
  \label{fig:comparison:DP}
\vspace{-5pt}
\end{figure*}
%%%--------------------------------------------------------------------------------
